Conditional Neural Architecture Search

Designing resource-efficient Deep Neural Networks (DNNs) is critical to deploy deep learning solutions over edge platforms due to diverse performance, power, and memory budgets. Unfortunately, it is often the case a well-trained ML model does not fit to the constraint of deploying edge platforms, causing a long iteration of model reduction and retraining process. Moreover, a ML model optimized for platform-A often may not be suitable when we deploy it on another platform-B, causing another iteration of model retraining. We propose a conditional neural architecture search method using GAN, which produces feasible ML models for different platforms. We present a new workflow to generate constraint-optimized DNN models. This is the first work of bringing in condition and adversarial technique into Neural Architecture Search domain. We verify the method with regression problems and classification on CIFAR-10. The proposed workflow can successfully generate resource-optimized MLP or CNN-based networks.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> refs.tex <==
@book{lamport94,
 author = "Leslie Lamport",
 title = "{\LaTeX: A Document Preparation System}",
 year = "1994",
 publisher = "Addison-Wesley",
 edition = "2nd",
 address = "Reading, Massachusetts"
}

@inproceedings{nicepaper1,
  author = "Firstname1 Lastname1 and Firstname2 Lastname2",
  title = "A Very Nice Paper To Cite",
  year = "2016",
  booktitle = "Proceedings of the 49th Annual IEEE/ACM International Symposium on Microarchitecture"
}

@inproceedings{nicepaper2,
  author = "Firstname1 Lastname1 and Firstname2 Lastname2 and Firstname3 Lastname3",
  title = "Another Very Nice Paper to Cite",
  year = "2015",
  booktitle = "Proceedings of the 48th Annual IEEE/ACM International Symposium on Microarchitecture"
}

@inproceedings{nicepaper3,
  author = "Firstname1 Lastname1 and Firstname2 Lastname2 and Firstname3 Lastname3 and Firstname4 Lastname4 and Firstname5 Lastname5 and Firstname6 Lastname6 and Firstname7 Lastname7 and Firstname8 Lastname8 and Firstname9 Lastname9 and Firstname10 Lastname10 and Firstname11 Lastname11 and Firstname12 Lastname12",
  title = "Yet Another Very Nice Paper To Cite, With Many Author Names All Spelled Out",
  year = "2011",
  booktitle = "Proceedings of the 38th Annual International Symposium on Computer Architecture"
}


==> sections/02-Background-orig.tex <==
\section{Relevant Background}
\TK{Plan is to merge Background and Related Work as there is heavy overlap. Alternately - give brief background of GAN and push rest to Related Work}


Resource constraints on edge-devices have led to active interest in DNN models which trade-off a little bit of accuracy for lower compute and memory footprint. We contrast our work to state-of-the-art related works in \autoref{table:compare_table}.


\subsection{Device-aware efficient Neural Architectures}

\textbf{Small DNN Models.} Smaller manually optimized DNN models 
like SqueezeNet \cite{squeezenet}, MobileNet \cite{sandler2018mobilenetv2}, and ShuffleNet \cite{zhang2018shufflenet} are popular examples.
To minimize human effort on designing the model, many current approaches apply multi-objective on meta-learning \cite{hochreiter2001learning, wong2018transfer} and Neural Architecture Search (NAS) \cite{mnasnet,hsu2018monas, he2018amc, dong2018dpp, elsken2018multi}  to optimize both performance and HW resources. 


% Constrained by resources, deploying the best performing model incurs high demand on storage and latency. The works on quantization and compressing technique strike the interest of DNN practitioners. Also, manually designed efficient models achieve good performance under embedded device sizes. To minimize the human effort on designing the model, many current researches apply multi-objective on meta-learning \cite{hochreiter2001learning, wong2018transfer} and Neural Architecture Search (NAS) \cite{mnasnet,hsu2018monas, he2018amc, dong2018dpp, elsken2018multi}  to optimize both performance and HW resources. The related works are summarized in \autoref{table:compare_table}.
%  This automation successfully bridges the gap between DNN model developers and EDA practitioners.
 
%  the upstream model design with downstream HW deployments together and decreases the exploring time for DNN practitioners to reach optimize deployed strategies.


% Our goal is to accelerate the DNN design loop from the defined problem to the Network configuration, fitting resource constraint. 


%\subsection{Manually designed %\TK{can be shortened - community knows what ASICs, FPGAs etc are. Move into Section 2.1}
%Edge devices are often composed of low-end processors and limited SRAM and DRAM. To accelerate DNNs, specialized hardware accelerators are being deployed to run DNNs with high throughput and energy efficiency. The platforms of DNN accelerators fall into three main categories: micro-controllers, Application Specific Integrated Circuits (ASICs), and Field Programmable Gate Arrays (FPGAs). For the edge-device DNN accelerator deployed in micro-controller and ASIC, we not only consider throughput and energy efficiency but also cost that leads to limited storage and computing power. Likewise, FPGAs are reconfigurable chips that packaged with fixed number of registers, Lookup Tables (LUTs), ans on-chip RAMs. For a hardware-friendly model, 
% many researches work on dataflow design to pipe the millions of parameter into the accelerator efficiently. 
%ome research works on manually designing a smaller models such as SqueezeNet \cite{squeezenet}, MobileNet \cite{sandler2018mobilenetv2}, and ShuffleNet \cite{zhang2018shufflenet}, where often requires empirical tuning and heuristic optimization. 

%\subsection{Quantization of DNN}
\textbf{DNN Quantization.}
Another category of work revolves around reducing the footprint of the model on the resultant hardware by quantizing the weights and activations of DNN to present the 32-bit floating number in lower bit-width \cite{courbariaux2015binaryconnect, rastegari2016xnor, zhou2017incremental}.
% such as Ternary weight networks, Binary Neural Networks, and XNOR-net. 
The quantized model, can both reduce the parameter size and minimize the inference time \cite{judd2016stripes}, a concept that is leverage by this work to achieve the reduce model size.
Many quantization techniques have been presented to performance quantization at inference time without performance degrade such as Deep Compression\cite{han2015deep}, Entropy-constrained scalar quantization \cite{choi2016towards}. However, they often require human effort to optimize the quantized bit-width of the model. To achieve aggressive quantization, many works apply the re-training to the quantized model \cite{zhou2017incremental, zhou2016dorefa}. On the other hand, Binarized Neural Network \cite{courbariaux2016binarized} and XNOR-Net \cite{rastegari2016xnor}, binarize both weight and activation so that the arithmetic can be replaced with bit-wise operation, using specialized hardware designs.
% However, quantization frameworks are often based on pre-trained full-precision models, which implying the model diversity is restricted.

% However, the model diversity of the inference quantization is restricted by the pre-trained model. On the other hand, trainable quantization increase the search space of the model and may reach better optimal points. Hence, quantized during training method, such as XNOR-Net \cite{rastegari2016xnor},DoReFa-Net \cite{zhou2016dorefa}, ABC-Net \cite{tang2017train}, is our focus in this investigation.

In this work, we target the platform of common edge devices, where floating point arithmetic is expensive, while integer operations are more hardware efficient. We follow the concept of integer-arithmetic-only quantization \cite{int_Quantize}, which presents all parameters arithmetic in integers. We follow a similar 
 technique to integrate the quantized behavior within the training loop. With this trainable quantization method, our model can learn the  network architecture and quantization bit-width at the same time.


% \TK{point to papers like Stripe (https://ieeexplore.ieee.org/document/7783722) and recent ones showing DNN accelerators for quantized models}

\subsection{Multi-objective NAS frameworks}

%\subsubsection{Methods of NAS}
Neural Architecture Search (NAS) automates the search process of the model for machine learning and deep learning. NAS has outperformed human designed architecture on  tasks such as image classification and object detection \cite{zoph2018learning, real2019aging}. Most of the  NAS works can be formulated as a hyper-parameter search problem. However, as the search space is extremely large there has been considerable work focusing on the development of techniques for efficient search of the hyper-parameters \cite{cai2018efficient, pham2018efficient}. The search methods include Bayesian optimization \cite{kandasamy2018neural, bergstra2013making, domhan2015speeding, mendoza2016towards}, reinforcement learning\cite{zoph2016neural, baker2016designing, zhang2018graph}, and genetic algorithms and evolution strategies \cite{stanley2019designing, jozefowicz2015empirical, stanley2002evolving}. Most of these approaches consume weeks of training \cite{cai2018proxylessnas} to reach the target objective. The objective function of these search methods are often formulated as a maximisation problem of model performance (e.g., accuracy), which leads a single point solution. It is important to note that the entire search process has to be repeated for a new hardware design problem, with each search taking weeks to complete, and there is little to no knowledge transferred across these designs.

%\subsubsection{Multi-objective NAS}
%\TK{This subsection could be moved to appendix.}
%While most NAS works are optimizing the accuracy, device-aware NAS \cite{mnasnet, tan2019efficientnet, kim2017nemo} jointly optimize accuracy and device constraint by adding the device constraint into the target function, called multi-objective optimization. MNAS \cite{mnasnet} considers the objective function of both accuracy and model latency to fit into mobile devices. MONAS \cite{hsu2018monas} incorporates power, and MAC operation constraints. In general, the objective function of constraint optimization can be formulated as:
%%  \begin{equation}\label{eq:eq1}
%%   \begin{multlined}
%% \max\limits_{m} Acc(m),\\
%% s.t.  \:  Storage(m) < S_{constaint} \\
%% s.t.  \:  Latency(m) < T_{constaint},
%%  \end{multlined}
%% \end{equation}

%\begin{flalign}
%\hskip\parindent & \begin{gathered}
%\max\limits_{m} Acc(m),\\
%s.t.  \:  Storage(m) < S_{constaint} \\
%s.t.  \:  Energy(m) < E_{constaint},
%    \end{gathered} &
%\end{flalign}

%which maximize the accuracy, constrained by the storage and energy. Acc is accuracy, m indicates model,  $S_{constaint}$ and  $E_{constaint}$ are the storage and energy constraint from the deployed platform, representing a sample set of the constraints that can be added to the optimization problem. There are many methods in the literature that are capable of handling such multi-object optimization problems \cite{marler2004survey}; one general method can be formulated as:
%%  \begin{equation}\label{eq:eq2}
%%   \begin{multlined}
%% \max\limits_{m} \alpha \: Acc(m) + \beta \: %Storage(m) + \gamma \: Latency(m),\\
%% s.t.  \:  \alpha + \beta + \gamma = 1,
%%  \end{multlined}
%% \end{equation}

%\begin{flalign}
%\hskip\parindent & \begin{gathered}
%\max\limits_{m} \alpha \: Acc(m) + \beta \: %Storage(m) + \gamma \: Energy(m),\\
%s.t.  \:  \alpha + \beta + \gamma = 1,
%    \end{gathered} &
%\end{flalign}

%in which the weighting parameters of $\alpha$, $\beta$, and $\gamma$ required manual tuning. As the number of constraints increases, the time for manual tuning of the weighting to find feasible objective function grows exponentially. Moreover, a optimization process on an set of weighting parameters takes weeks of training, which becomes a time-consuming task when the iterative tuning of the weighting parameters is required.

%For adapting to different platform, MNAS \cite{mnasnet} generates multiple data points on the Pareto frontier after one launch of search, which gives more diverse neural architecture. However, those data points are centered in a narrow range of accuracy level, which is closely-correlated with the weighting of the constraint in multi-objective function. It implies if we train the neural architecture search to emphasize on high accuracy, even though those different architecture may be feasible for some platforms, it is hard to transfer the learned data points to lower-end platforms that are highly resource-constrained. In practice, when the constraint changes, it is necessary to execute the search once more along with the identification of the appropriate hyper-parameters. 

%These multi-objective NAS approaches however are still one step away from our goal, to provide transferable device-aware model without the retraining overhead. We categorize them into three challanges: 1) the manual tuning weighting between different constraint; 2) the range of resultant data points is limited according to the fixed objective function \cite{mnasnet} ; 3) weeks of retraining when changing deployed device. 

%% First, NASs often take weeks of training to fit the designed objective function \cite{cai2018proxylessnas}. Once the objective function changes, the search needs to be relaunched. Second, given the high computation cost, some works save multiple Pareto-optimal solutions \cite{mnasnet} for different HW requirements. However, the data points generated from the Pareto frontier are often with high likelihood owing to the fixed objective function. It is hard to mitigate to different HW requirements. Third, the multi-objective training require weighting of different constraints, where the manual tuning of the constraint lead to different Pareto frontier. 


\subsection{Generative Adversarial Networks (GAN)}
Generative Adversarial Nets (GANs) \cite{goodfellow2014generative} and Variational autoencoders (VAEs) \cite{VAE} are two most prominent generative models for synthesizing images. VAEs maximize a variational lower bound on the log-likelihood of the training data and VAEs are trained to synthesize data with good log-likelihood to the original dataset. Orthogonally GANs, based on game theory approach, contains a generative network (\textit{generator}) and adversarial network (\textit{discriminator}). The generative model is pitted against the discriminator, which learns to determine whether a sample is from generator or training data. They are both trained iteratively to outperform each other, and resulting in both models improving over the course of the training process. The generator's goal is to learn the mapping from the distribution of latent space to the distribution of the data space. The discriminator's goal is to maximize its ability to identify synthesized data. 

Instead of building multiple GAN networks for different class of images, the fundamental GAN can be augmented by incorporating side information (class) \cite{mirza2014conditional, van2016conditional}. Both the generator and discriminator take in the class label in the training phase, so that the mapping of class label to the distribution of different class can be learned. In other branches of a similar approach, such as ACGAN \cite{acgan}, infoGAN \cite{infogan}, and others \cite{odena2016semi, ramsundar2015massively}, rather than feeding in side-information to discriminator, the discriminator is tasked to reconstruct the class label, which is taken by the generator. GAN frameworks have been successfully applied to other tasks such as language processing \cite{press2017language} and regression problem \cite{rezagholiradeh2018reg}.

This paper is the first, to the best of our knowledge, to extend the GAN framework for the task of NAS, which instantly samples the models from the distribution that is conditioned by different objectives, e.g., accuracy, without the re-searching process of the related NAS frameworks, as shown in \autoref{fig:compare}. 



\begin{figure}
\centering
\subfigure[NAS-related methods]{\includegraphics[width=1\linewidth]{Figures/compare_a.pdf}}
\subfigure[NAGAN Approach]{\includegraphics[width=0.8\linewidth]{Figures/compare_b.pdf}}
\caption{NAS-related methods require weeks of searching time for proposals, optimized by each targeted performance. In contrast, NAGAN generates the the proposals, conditioned on each targeted performance within seconds.}
\label{fig:compare}
\end{figure}




==> sections/05-CaseStudy.tex <==
\section{Case Study}
Extension of same framework to different hyperparameter
\subsection{quantization bit of Resnet, Mobilenet}
\subsection{pruning strategy for Resnet, Mobilenet}


==> sections/07-Discussion.tex <==
%\section{Discussion and Future work}

\subsection{Discussion and Future work}

\textbf{More descriptive representations of the network.}
We use the network descriptor with nodes per layer and bits per layer. However, more descriptions can be Incorporated to genereate richer representations of the network. For example, we could enable pruning by adding pruning percentage per layer. We could also tune more model hyper-parameter such as types of activation function, dropout rate, number of epochs and learning rate. While these provides a more complete representation of the network, they increase the search space and the complexity that the GAN would have to encounter. There may be new considerations that have to be incorporated into the training of the generator to capture the increase in complexity.

\textbf{Pruning and quantization from pre-trained model.}
We expect the developed framework can be applied to optimize the pre-trained model by learning the pruning and quantization strategy. The presented generative method could be an alternative to the reinforcement learning-based methods \cite{he2018amc, wang2019haq} to compress DNN model.

\textbf{Electronics Design Autonomy.}
We expect the full automation of hardware deployment, which minimizes the effort required from a EDA engineer completely automating the hardware deployment process. We expect the device-aware neural network description generated from INAG to be an input of ML high level synthesis EDA tools \cite{duarte2018fast}, in our future work. Finally, after the generative model is tuned and trained by ML experts, the hardware-optimized neural network could be automatically deployed. 

We leave these three directions as our future work.
% On the other hand, we could also fix the number of nodes per layer and only tune the quantization bit-width. This could be a useful usecase for some existing manually designed models, which the pre-trained weights on large dataset is available such as MobileNetv2 \cite{sandler2018mobilenetv2} and YOLOv3 \cite{redmon2018yolov3}. We could initialize with pre-trained weight and only train to learn the best quantization strategies. We leaves these two directions as our future works.

% \subsection{network description to FPGA/ASIC automation}
% The ultimate goal of this investigation is to decrease the turn-around time from developing DNN structure for defined problems to edge-device or HW deployment. The INAG outputs a network descriptor which could dictate the HW deployment such as the implementation on FPGA or ASIc. We aim to automate the path from network descriptor to FPGA/ASIC implementation as well to achieve the final workflow as: an ML practitioner with a trained NAGAN specifies the device constraint, and INGM workflow can lead to configured device automatically. We leaves this as another branch of our future works.
% \subsection{Put the storage latency in to constraint}

==> table/error_v0.tex <==
\begin{table}[]
\caption{The evaluation of generator.}
\begin{tabular}{ccccccc}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}Arch.} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}MLP} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}CNN} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}Prob.} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}Regrssion} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}Classification} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}Data} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}$Data_{a}$} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}$Data_{b}$} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}CH} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}MNIST} & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}CIFAR-10} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Exp.\\ Name\end{tabular}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Reg.A}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Reg.B}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Reg.C}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Cls.A}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Cls.B}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{Cls.C}} \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}$Err_{f}$} & \multicolumn{1}{c|}{0.3} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{0.5} & \multicolumn{1}{c|}{0.3} & \multicolumn{1}{c|}{0.4} & \multicolumn{1}{c|}{4.8} \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}$Err_{r}$} & \multicolumn{1}{c|}{12.0} & \multicolumn{1}{c|}{6.2} & \multicolumn{1}{c|}{11.3} & \multicolumn{1}{c|}{8.1} & \multicolumn{1}{c|}{11.7} & \multicolumn{1}{c|}{8.7} \\ \hline
\multicolumn{7}{l}{}
\end{tabular}
\label{table:error}
\end{table}





% \begin{table}[]
% \begin{tabular}{ccccccc}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}Arch.} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}MLP} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}CNN} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}Prob.} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}Regrssion} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}Classification} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}Data} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}$Data_{1}$} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}$Data_{2}$} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}C.H.} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}MNIST} & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}CIFAR} \\ \hline
% \multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}$Err_{f}$} & \multicolumn{1}{c|}{0.3} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{0.5} & \multicolumn{1}{c|}{0.3} & \multicolumn{1}{c|}{0.4} & \multicolumn{1}{c|}{17.8} \\ \hline
% \multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}$Err_{r}$} & \multicolumn{1}{c|}{12.0} & \multicolumn{1}{c|}{6.2} & \multicolumn{1}{c|}{11.3} & \multicolumn{1}{c|}{8.1} & \multicolumn{1}{c|}{11.7} & \multicolumn{1}{c|}{26.9} \\ \hline
% \multicolumn{7}{l}{$Err_{f}$, $Err_{r}$ (\%)}
% \end{tabular}
% \caption{The generator error of experiments.}
% \label{table:error}
% \end{table}

% \begin{table}[]
% \begin{tabular}{ccccccc}
% \hline
% \multicolumn{1}{|c|}{Arch.} & \multicolumn{5}{c|}{MLP} & \multicolumn{1}{c|}{CNN} \\ \hline
% \multicolumn{1}{|c|}{Prob.} & \multicolumn{3}{c|}{Regrssion} & \multicolumn{3}{c|}{Classification} \\ \hline
% \multicolumn{1}{|c|}{Data} & \multicolumn{1}{c|}{$Data_{1}$} & \multicolumn{1}{c|}{$Data_{2}$} & \multicolumn{1}{c|}{C.H.} & \multicolumn{1}{c|}{MNIST} & \multicolumn{2}{c|}{CIFAR} \\ \hline
% \multicolumn{1}{|c|}{$Err_{f}$} & \multicolumn{1}{c|}{0.3} & \multicolumn{1}{c|}{1.2} & \multicolumn{1}{c|}{0.5} & \multicolumn{1}{c|}{0.3} & \multicolumn{1}{c|}{0.4} & \multicolumn{1}{c|}{17.8} \\ \hline
% \multicolumn{1}{|c|}{$Err_{r}$} & \multicolumn{1}{c|}{12.0} & \multicolumn{1}{c|}{6.2} & \multicolumn{1}{c|}{11.3} & \multicolumn{1}{c|}{8.1} & \multicolumn{1}{c|}{11.7} & \multicolumn{1}{c|}{26.9} \\ \hline
% \multicolumn{7}{l}{$Err_{f}$, $Err_{r}$ (\%)}
% \end{tabular}
% \caption{The generator error of experiments.}
% \label{table:error}
% \end{table}



==> table/exp_table_old.tex <==
% Please add the following required packages to your document preamble:

\begin{table*}[]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 &  & \textbf{Perf.} & \textbf{Storage} & \textbf{Energy} & \textbf{Time} & \textbf{Arch} \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Target Perf 100\%\\ Const\end{tabular}}} & \textbf{GA} & 97.3 & 20.7 & 21.0 &  & (42,59,62),(7,5,4,6) \\ \cline{2-7} 
 & \textbf{Bayesian} & 97.7 & 20.2 & 21.3 &  & (55,11,21), (4,12,3,5) \\ \cline{2-7} 
 & \textbf{NAGAN} & 95 & 19.7 & 19.6 &  & (63,57,13),(4,4,15,16) \\ \hline
\textbf{Target Perf. 75\%} & \textbf{NAGAN} & 73 & 1.9 & 1.5 &  & (19, 13, 17), (4,3,3,16) \\ \hline
\textbf{Target Perf. 50\%} & \textbf{NAGAN} & 48.6 & 0.6 & 0.5 &  & (5,8,14), (5,3,4,5) \\ \hline
\textbf{Target Perf. 25\%} & \textbf{NAGAN} & 24.4 & 0.5 & 0.4 &  & (3,6,12), (15,4,3,4) \\ \hline
\textbf{Target Perf. 75\%} & \textbf{NAGAN} & 73 & 1.4 & 1.2 &  & (18,18,18), (3,2,2,16) \\ \hline
\end{tabular}
\caption{The comparisons of NAGAN,  GA, and Bayesian on experiment setting 1.}
\label{table:exp_table}
\end{table*}

==> table/exp_table_old2.tex <==
% Please add the following required packages to your document preamble:

% \begin{table*}[]
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{2}{|c|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}Exp. Setting 1} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}Exp. Setting 2} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{2}{|c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Constraint\\ (Storage, Energy)\end{tabular}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Target Perf.: P\_\{max\}\\ (S. \textless{}20\%, E. \textless{}20\%)\end{tabular}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Target Perf.: P\_\{max\}\\ (S. \textless{}13\%, E. \textless{}13\%)\end{tabular}} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
%  & \begin{tabular}[c]{@{}c@{}}Training \\ size (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Perf.\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Storage\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Perf.\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Storage\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy\\ (\%)\end{tabular} \\ \hline
% \cellcolor[HTML]{EFEFEF}\textbf{GA} & 100 & 97.3 & 20.7 & 21.0 & 69.5 & 11.5 & 11.5 \\ \hline
% \cellcolor[HTML]{EFEFEF}\textbf{Bayseian} & 100 & 97.7 & 20.2 & 21.3 & 69 & 12.2 & 12.2 \\ \hline
% \cellcolor[HTML]{EFEFEF} & 100 & 95 & 19.7 & 19.6 & 58 & 12.9 & 12.9 \\ \cline{2-8} 
% \cellcolor[HTML]{EFEFEF} & 70 & 95 & 18.8 & 17.9 & 51 & 12.7 & 12 \\ \cline{2-8} 
% \cellcolor[HTML]{EFEFEF} & 33 & 93 & 14.7 & 13.2 & 50 & 11.6 & 11.2 \\ \cline{2-8} 
% \multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\textbf{INAG}} & 5 & 24.4 & 15.6 & 15.4 & 40 & 12.6 & 12.1 \\ \hline
% \end{tabular}
% \caption{The comparisons of NAGAN,  GA, and Bayesian on experiment setting 1 and 2.}
% \label{table:exp_table}
% \end{table*}


% Please add the following required packages to your document preamble:

\begin{table*}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{|c|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}Exp. Setting 1} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}Exp. Setting 2} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{2}{|c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Constraint\\ (Storage, Energy)\end{tabular}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Target Perf.:$P_{max}$\\ (S. \textless{}21\%, E. \textless{}21\%)\end{tabular}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Target Perf.: $P_{max}$\\ (S. \textless{}13\%, E. \textless{}13\%)\end{tabular}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
 & Training size (\%) & Perf.(\%) & Storage(\%) & Energy(\%) & Perf.(\%) & Storage(\%) & Energy(\%) \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{GA} & 100 & 97.3 & 20.7 & 21.0 & 69.5 & 11.5 & 11.5 \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Basiean} & 100 & 98.7 & 20.2 & 21.3 & 66 & 12.2 & 12.2 \\ \hline
\cellcolor[HTML]{EFEFEF} & 100 & 95 & 19.7 & 19.6 & 58 & 12.9 & 12.9 \\ \cline{2-8} 
\cellcolor[HTML]{EFEFEF} & 70 & 95 & 18.8 & 17.9 & 51 & 12.7 & 12 \\ \cline{2-8} 
\cellcolor[HTML]{EFEFEF} & 33 & 93 & 14.7 & 13.2 & 50 & 11.6 & 11.2 \\ \cline{2-8} 
\cellcolor[HTML]{EFEFEF} & 5 & 91 & 15.6 & 15.4 & 40 & 12.6 & 12.1 \\ \cline{2-8} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & Training size (\%) & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Target Perf.: $P_{max}$\\ (S. \textless{}6\%, E. \textless{}6\%)\end{tabular}} & \multicolumn{3}{c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Target Perf.: 75\%$P_{max}$\\ (S. \textless{}10\%, E. \textless{}10\%)\end{tabular}} \\ \cline{2-8} 
\multirow{-6}{*}{\cellcolor[HTML]{EFEFEF}\textbf{INAG}} & 100 & 91 & 5.6 & 5.1 & 40 & 9.1 & 8.5 \\ \hline
\end{tabular}
\caption{The comparisons of NAGAN,  GA, and Bayesian on experiment setting 1 and 2.}
\label{table:exp_table}
\end{table*}




% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[]
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{2}{|c|}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{4}{c|}{\cellcolor[HTML]{EFEFEF}Exp. Setting 1} & \multicolumn{4}{c|}{\cellcolor[HTML]{EFEFEF}Exp. Setting 2} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{2}{|c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Constraint\\ (Storage, Energy)\end{tabular}} & \multicolumn{4}{c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Target Perf.: P\_\{max\}\\ (S. \textless{}21\%, E. \textless{}21\%)\end{tabular}} & \multicolumn{4}{c|}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Target Perf.: P\_\{max\}\\ (S. \textless{}13\%, E. \textless{}13\%)\end{tabular}} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
%  & \begin{tabular}[c]{@{}c@{}}Training \\ size (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Perf.\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Storage\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy\\ (\%)\end{tabular} & Time & \begin{tabular}[c]{@{}c@{}}Perf.\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Storage\\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Energy\\ (\%)\end{tabular} & Time \\ \hline
% \cellcolor[HTML]{EFEFEF}\textbf{GA} & 100 & 97.3 & 20.7 & 21.0 &  & 69.5 & 11.5 & 11.5 &  \\ \hline
% \cellcolor[HTML]{EFEFEF}\textbf{Basiean} & 100 & 97.7 & 20.2 & 21.3 &  & 69 & 12.2 & 12.2 &  \\ \hline
% \cellcolor[HTML]{EFEFEF} & 100 & 95 & 19.7 & 19.6 &  & 58 & 12.9 & 12.9 &  \\ \cline{2-10} 
% \cellcolor[HTML]{EFEFEF} & 70 & 95 & 18.8 & 17.9 &  & 51 & 12.7 & 12 &  \\ \cline{2-10} 
% \cellcolor[HTML]{EFEFEF} & 33 & 93 & 14.7 & 13.2 &  & 50 & 11.6 & 11.2 &  \\ \cline{2-10} 
% \multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\textbf{INAG}} & 5 & 24.4 & 15.6 & 15.4 &  & 40 & 12.6 & 12.1 &  \\ \hline
% \end{tabular}
% \end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
%  & \textbf{\begin{tabular}[c]{@{}c@{}}Training \\ size\end{tabular}} & \textbf{Perf.} & \textbf{Storage} & \textbf{Energy} & \textbf{Time} & \textbf{\begin{tabular}[c]{@{}c@{}}Netw. Desc.\\ (Nodes), (Bits)\end{tabular}} \\ \hline
% \textbf{GA} & 100\% & 97.3 & 20.7 & 21.0 &  & (42,59,62,1), (7,5,4,6) \\ \hline
% \textbf{Basiean} & 100\% & 97.7 & 20.2 & 21.3 &  & (55,11,21,1), (4,12,3,5) \\ \hline
% \multirow{4}{*}{\textbf{INAG}} & 100\% & 95 & 19.7 & 19.6 &  & (63,57,13,1), (4,4,15,16) \\ \cline{2-7} 
%  & 70\% & 95 & 18.8 & 17.9 &  & (56,53,31,1), (13,5,5,5) \\ \cline{2-7} 
%  & 33\% & 93 & 14.7 & 13.2 &  & (42,14,64,1), (10,3,16,16) \\ \cline{2-7} 
%  & 5\% & 24.4 & 15.6 & 15.4 &  & (17,43,26,1), (3,3,16,16) \\ \hline
% \end{tabular}
% \end{table}


% \begin{table*}[]
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
%  & \textbf{\begin{tabular}[c]{@{}c@{}}Training \\ size\end{tabular}} & \textbf{Perf.} & \textbf{Storage} & \textbf{Energy} & \textbf{Time} & \textbf{\begin{tabular}[c]{@{}c@{}}Netw. Desc.\\ (Nodes), (Bits)\end{tabular}} \\ \hline
% \textbf{GA} & 100\% & 97.3 & 20.7 & 21.0 &  & (42,59,62,1), (7,5,4,6) \\ \hline
% \textbf{Basiean} & 100\% & 97.7 & 20.2 & 21.3 &  & (55,11,21,1), (4,12,3,5) \\ \hline
% \multirow{4}{*}{\textbf{INAG}} & 100\% & 95 & 19.7 & 19.6 &  & (63,57,13,1), (4,4,15,16) \\ \cline{2-7} 
%  & 70\% & 95 & 18.8 & 17.9 &  & (56,53,31,1), (13,5,5,5) \\ \cline{2-7} 
%  & 33\% & 93 & 14.7 & 13.2 &  & (42,14,64,1), (10,3,16,16) \\ \cline{2-7} 
%  & 5\% & 24.4 & 15.6 & 15.4 &  & (17,43,26,1), (3,3,16,16) \\ \hline
% \end{tabular}
% \caption{The comparisons of NAGAN,  GA, and Bayesian on experiment setting 1.}
% \label{table:exp_table}
% \end{table*}

==> table/exp_table_reg3.tex <==
% Please add the following required packages to your document preamble:

\begin{table*}[]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 &  & \textbf{Perf.} & \textbf{Storage} & \textbf{Energy} & \textbf{Time} & \textbf{Arch} \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Target Perf 100\%\\ Const\end{tabular}}} & \textbf{GA} & 69.5 & 11.5 & 11.5 &  & (43,61,53),(2,2,3,7) \\ \cline{2-7} 
 & \textbf{Bayesian} & 69 & 12.2 & 12.2 &  & (55,11,21), (4,12,3,5) \\ \cline{2-7} 
 & \textbf{NAGAN} & 58 & 12.9 & 12.9 &  & (64,63,64),(2,2,2,13) \\ \hline
\textbf{Target Perf. 75\%} & \textbf{NAGAN} & 40 & 12 & 11.2 &  & (35, 39, 39), (11,5,5,5) \\ \hline
\textbf{Target Perf. 50\%} & \textbf{NAGAN} & 26.9 & 7.6 & 7 &  & (33,25,38), (10,5,5,4) \\ \hline
\textbf{Target Perf. 25\%} & \textbf{NAGAN} & 13.5 & 3.5 & 3.2 &  & (22,21,26), (5,4,4,5) \\ \hline
\end{tabular}
\caption{The comparisons of NAGAN,  GA, and Bayesian on experiment setting 2.}
\label{table:exp_table_reg3}
\end{table*}

==> table/exp_table_v0.tex <==
\begin{table*}[]
\caption{The comparisons of INAG,  GA, and Bayesian on Reg.A and Reg.B under a certain constraint(Cstr. A).}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
 & \multicolumn{4}{c|}{\cellcolor[HTML]{EFEFEF}Reg. A} & \multicolumn{4}{c|}{\cellcolor[HTML]{EFEFEF}Reg. B} \\ \hline
\rowcolor[HTML]{C0C0C0} 
Cstr. A & \multicolumn{4}{c|}{\cellcolor[HTML]{C0C0C0}Target Perf.:  $P_{max}$(S. \textless{}21\%, E. \textless{}21\%)} & \multicolumn{4}{c|}{\cellcolor[HTML]{C0C0C0}Target Perf.:  $P_{max}$(S. \textless{}13\%, E. \textless{}13\%)} \\ \hline
\rowcolor[HTML]{EFEFEF} 
 & Perf.(\%) & Storage(\%) & Energy(\%) & Search Time & Perf.(\%) & Storage(\%) & Energy(\%) & Search Time \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{GA} & 97.3 & 20.7 & 21.0 & 6 hrs & 69.5 & 11.5 & 11.5 & 6 hrs \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Bayesian} & 97.7 & 20.2 & 21.3 & 13 hrs & 66 & 12.2 & 12.2 & 13 hrs \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{INAG} & 95 & 19.7 & 19.6 & 5 secs & 58 & 12.9 & 12.9 & 5 secs \\ \hline

\end{tabular}
\label{table:exp_table}
\end{table*}

==> table/exp_table_v1.tex <==
\begin{table}[]
\caption{The comparisons of INAG,  GA, and Bayesian on Reg.A and Reg.B under a certain constraint(Cstr. A).}
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
 & \multicolumn{4}{c|}{\cellcolor[HTML]{EFEFEF}Reg. A} \\ \hline
\rowcolor[HTML]{C0C0C0} 
Cstr. A & \multicolumn{4}{c|}{\cellcolor[HTML]{C0C0C0}Target Perf.:  $P_{max}$(S. \textless{}21\%, E. \textless{}21\%)}  \\ \hline
\rowcolor[HTML]{EFEFEF} 
 & Perf.(\%) & Storage(\%) & Energy(\%) & Search Time  \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{GA} & 97.3 & 20.7 & 21.0 & 6 hrs  \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{Bayesian} & 97.7 & 20.2 & 21.3 & 13 hrs \\ \hline
\cellcolor[HTML]{EFEFEF}\textbf{INAG} & 95 & 19.7 & 19.6 & 5 secs \\ \hline

\end{tabular}
\label{table:exp_table}
\end{table}

==> table/s3.tex <==
\begin{table}[]
\scalebox{0.7}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
          & \multicolumn{3}{c|}{GA}    & \multicolumn{3}{c|}{PEPG}  & \multicolumn{3}{c|}{CMAES}  \\ \hline
          & $Ep_{0}$ & $Ep_{50}$ & Impr. & $Ep_{0}$ & $Ep_{50}$ & Impr. & $Ep_{0}$ & $Ep_{50}$ & Impr.  \\ \hline
Tornado    & 4.35  & 4.53       & +4.66 & 4.16  & 4.35       & +4.57 & 4.19  & 4.62       & +10.26 \\ \hline
Shuffle    & 5.88  & 6.13       & +4.25 & 6.27  & 5.83       & +7.55 & 5.90  & 6.23       & +5.60  \\ \hline
BitReverse & 4.94  & 5.02       & +1.74 & 4.93  & 5.17       & +4.87 & 4.94  & 5.13       & +3.88  \\ \hline
BitRotate  & 6.44  & 6.55       & +1.72 & 6.13  & 6.6        & +7.67 & 6.35  & 6.51       & +2.55  \\ \hline
Neighbor   & 14.81 & 15.12      & +2.10 & 15.03 & 15.33      & +2.03 & 14.20 & 15.08      & +6.20  \\ \hline
Uniform    & 4.80  & 4.83       & +0.62 & 4.79  & 4.84       & +1.04 & 4.79  & 4.84       & +1.04  \\ \hline
\end{tabular}}
 \vspace{0.30cm}
\caption{Throughput of the NoC with EA-based VC allocation in different traffic from gem5}
 \vspace{-0.30cm}
\label{table:s3}
\end{table}

==> table/s4.tex <==
% \begin{table}[]
% \scalebox{0.7}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \hline
%           & \multicolumn{3}{c|}{GA}     & \multicolumn{3}{c|}{PEPG}  & \multicolumn{3}{c|}{CMAES}  \\ \hline
%           & $Ep_{0}$  & $Ep_{50}$ & Impr. & $Ep_{0}$ & $Ep_{50}$ & Impr. & $Ep_{0}$  & $Ep_{50}$ & Impr. \\ \hline
% BC        & 25.56  & 25.61     & -0.19 & 25.76 & 25.72      & -0.16 & 25.56  & 25.57      & -0.08 \\ \hline
% BFSCC     & 25.60 & 25.58     & -0.09 & 25.64 & 25.62      & -0.07 & 25.63 & 25.58      & -0.18 \\ \hline
% Component & 25.39  & 25.36     & -0.13 & 25.43 & 25.37      & -0.24 & 25.44 & 25.45      & -0.35 \\ \hline
% BFS       & 25.54 & 25.51     & -0.12 & 25.80 & 25.66      & -0.54 & 25.61 & 25.46      & -0.50 \\ \hline
% kcore     & 25.96  & 25.68      & -1.09 & 25.66 & 25.61      & -0.19 & 25.64 & 25.566     & -0.28 \\ \hline
% PageRank  & 25.386 & 25.332     & -0.21 & 25.61 & 25.56      & -0.19 & 25.62  & 25.58      & -0.16 \\ \hline
% Radii     & 25.32 & 25.26     & -0.21 & 25.36 & 25.33      & -0.12 & 25.32 & 25.262     & -0.21 \\ \hline
% \end{tabular}}
% \vspace{0.30cm}
% \caption{Latency reduce of NoC with ES-based VC allocation in different traffic}
% \label{table:s4}
% \vspace{-0.30cm}
% \end{table}

==> table/time.tex <==

% \begin{table}[]
% \begin{tabular}{|c|c|c|c|c|}
% \hline
%                                                   & $\mathbf{Time_{S1}}$ & $\mathbf{Time_{S2_Tr}}$ & $\mathbf{Time_{S2_VC}}$ & $\mathbf{Time_{S3}}$ \\ \hline
% QL                                        & 178.1                                  & 137.6                                 & $N/A$                                  & $N/A$                       \\ \hline
% SARSA                                     & 162.0                                  & \textbf{133.6}                                  & $N/A$                                  & $N/A$                        \\ \hline
% E-SARSA                                            & 173.4                        & 139.9                         & $N/A$                                 & $N/A$                      \\ \hline
% \multicolumn{1}{|c|}{GA}   & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{l|}{147.2}             & 140.6                        \\ \hline
% \multicolumn{1}{|c|}{PEPG}   & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{l|}{147.4}             & 140.2                        \\ \hline
% \multicolumn{1}{|c|}{CMAES} & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{c|}{$N/A$}             & \multicolumn{1}{l|}{147.6}            & \textbf{133.8}                        \\ \hline
% \end{tabular}
% \vspace{0.30cm}
% \caption{The cost of training time (Seconds) for different policy learning techniques over interconnect environment for single iteration }
% \vspace{-0.30cm}
% \label{table:time}
% \end{table}
% \vspace{-0.3cm}
